An Image-based Typology for Visualization

We present and discuss the results of a qualitative analysis of visualization images to derive an image-based typology of visualizations. For each image, we seek to identify its main focus or the essential stimuli. As a result, we derived 10 image-based visualization types. We describe coding decisions we made in the derivation process. The resulting image typology can serve a number of purposes: enabling researchers and practitioners to identify visual design styles, facilitating the categorization of visualization images for the purpose of research and teaching, enabling researchers to study the evolution of the community and its research output over time, and facilitating a discussion of standardization in visualization. In addition, the tool and dataset enable scholars to closely examine the images and how they are published and communicated in our community. osf.io/dxjwt presents a pre-registration and all supplemental materials.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> TableImagesKeywordsStat.tex <==
\label{sec:dataset}
\begin{table}[!htb]
  \caption{Number of papers/number of figures per year per conference track, and 
  percentage of papers with keywords ($\%$ w/ keyW) every five years from 1990--2020. In the keywords related analysis,
  we use data from 2000--2020 due to scarce data points in
  the first two years. 
  }
  \label{tab:paperfigures}
  \scriptsize%
	\centering%
  \begin{tabu}{%
	m{0.1cm}%
	m{0.6cm}m{0.6cm}m{0.6cm}m{0.6cm}
	m{0.6cm}m{0.6cm}m{0.6cm}m{0.6cm}
	%*{8}{c}%
	}
  \toprule
   \rotatebox{90}{year} & \rotatebox{90}{Vis/SciVis} &   \rotatebox{90}{SciVis conf} & \rotatebox{90}{InfoVis} & \rotatebox{90}{InfoVis conf} &   \rotatebox{90}{VAST} &   \rotatebox{90}{VAST conf} &  Sum & \rotatebox{90}{$\%$ w/ keyW} \\
  \midrule
'20 & 32/374 &        & 65/614 & & 51/469 & 10/109 & 160/1566 &  \\
'15 & 33/401 & 9/80   & 38/387 & & 33/308 & 14/113 & 127/1289 &  \\
'10 & 48/575 &      & 35/318 & &  & 26/190 &  109/1083 &  \\
'05 &  & 88/847 &  & 31/296 & & & 119/1143 &  \\
'00 &  & 73/675  &  & 20/137  &   &  & 93/812 & \\
'95 &  & 56/424  &  & 18/97 &   &  & 74/521\\
'90 &  & 52/426  &  &  &   &  & 52/426  \\
  \midrule
  \textbf{sum} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{--} &\\
  \bottomrule
  \end{tabu}%
\end{table}

==> VisTypes/13vc.color.tex <==


\setlength{\pictureheight}{2.1cm}
\begin{figure}[h!]
\centering
%\hfil
%\subfloat[]{
\vspace{-1ex}
\includegraphics[clip, trim={350 60 0 20}, height=\pictureheight]{FigureVCExamples/color/VisJ.1457.8.jpg}\hfill%%
\includegraphics[clip, trim={50 20 780 100},height=\pictureheight]{FigureVCExamples/color/VASTJ.828.8.jpg}\hfill%%
%\label{fig:pa}}
%\subfloat[]{
\includegraphics[clip, trim={500 0 0 0},height=\pictureheight]{FigureVCExamples/color/VisJ.1547.6.jpg}\hfill%%
%\label{fig:fp}}
%\subfloat[]{
\includegraphics[clip, trim={50 80 50 70}, height=\pictureheight]{FigureVCExamples/color/InfoVisJ.1184.1.jpg}%
%\hfil
%\caption{}
\vspace{-2ex}
\label{fig:color}
\end{figure}


==> VisTypes/14vc.other.tex <==


This category includes anything that did not fit in any other category in our typology. 
%We used this category to describe what we saw preferably without using comments about what the data is about but rather about what the encoding looks like. \tomo{that is true for all categories, no?} 
We used this category to describe what we saw preferably without using comments about what the data is about but rather about what the encoding looks like that is not in the 13 types above. %\tomo{that is true for all categories, no?} 
general photographs potentially without annotations or labels (otherwise, it would be a schematic) ($\approx 200$ times), 
tables ($\approx 70$ times), plain text such as code, algorithms, texts that do not belong to the \vistext category ($\approx 20$ times), infographics, 
models, and legends (often color legends). 
%Photos can depict 2D or 3D scenes, and were coded accordingly.
%All photos are not necessarily 2D.\ms{weird formulation. Clear to us but likely not the reader?}


==> VisTypes/Challenges.tex <==

Challenging cases of generalized bar chart:
\begin{enumerate}
\setlength\itemsep{0em}
    \item Boxplots give evidence to the statistical description, where line length is essential to understanding. The line in a dot-plot also represents stack-together points. These points are linearly mapped to the range. 
    \item
    If only the bar top is shown (e.g., point-plot and Boxplot), use line \& point. If bars are drawn, use bar \& point. 
\end{enumerate}


==> VisTypes/MultiComposition.tex <==

Images that show a composition of multiple charts in a way that facilitates communication or rapid comparisons in subfigures. It could be a number of different data fields, using numerous encoding channels such as positioning in the coordinate (x, y), size, color, shape, etc. or many charts partitioning data into the same encodings in multiple charts.

\subsubsection{Yes, manually-arranged (for the purpose of communication / publication)}
Images containing (labeled or unlabeled) subfigures or insets on top of images. 
Callouts are manually arranged.

\subsubsection{Yes, machine-arranged (as part of the vis system/interface)}
The views are shown side-by-side as part of a visualization or visualization system. This may include multiple GUIs containing multiple visualizations or screenshots of a subset of a multiview system.  The view often has its own widgets and GUI components. \ms{Frankly, I am still confused by this reasoning. I am not sure if I had any situation in which I had multiple screenshots of a GUI that were machine arranged (multiple yes, but manually arranged). On the other hand, it is still not ``intuitive'' for me why we did not code multiview GUIs as multiview.}

\subsubsection{No (just one vis)}
When the view just has one visualization  but also single GUIs that might contain multiple windows / overlays as part of the same system.\ms{iirc the guideline was that every GUI (of a single tool) is automatically just one vis ... }
Also, if a schematic includes multiple different VIS examples and is just one schematic (\eg not multiple schematics side by side), it is not multiple views.


==> VisTypes/MultiNestedLayered.tex <==
Images containing layered / superimposition (multiple vis on top of each other) or nested (one vis representation inside another). Here the layered can mean the 2D/3D space or 2D/3D manifold space. 
It has at least two encoding techniques, such as wireframe mesh on top of a surface,
\eg, a cushion treemap (nested because of the shading and treemap together, not because of the containment relationships), 
painterly vector field (layered because of the vector glyph and the vorticity).

A single image
``multiple figures composed manually'' as a nested, \eg, call-out
subfigures containing a depiction of part of another subfigure
Containment relationships as nested due to data or algorithm, \eg, tree structures of a single encoding.
Small-multiples (they are ``data dimensionality'', not ``layout'')
Highlight or the photo category



==> VisTypes/dim3d.tex <==
3D representation has specific depth cues, such as shading, perspective, and lighting. It requires continuous 3D, rather than discrete layers for aesthetics or callout uses. Here, we ignore the media used to present the data. Thus a photo, a 3D data physicalization, and a desktop 3D interface can be 3D. 


==> fig.learningAssociation.tex <==



\begin{figure}[!tp]
  \centering  
  \includegraphics[width=\columnwidth]{figures/05_InfoVisC_149_10_imgnet.png}
%  \vspace{-.3ex}
 \caption{\tochange{\textbf{Instance-based search}. Model prediction to recommend similar images in our dataset.
 When model is presented with the top-left image, it shows the similarity distribution scores (top-right) and recommended the five most (mid-row) and five least similar image (bottom-row). 
 }}
   \label{fig:learningAssociation}
\end{figure}



==> fig.visTypesNet.tex <==

\begin{figure*}[!tp]
  \centering  
  \includegraphics[width=0.5\textwidth]{figures/supervised_weights_s66_umap.png}
%  \vspace{-.3ex}
 \caption{\tochange{\modelname: A two-dimensional U-MAP projection of the dataset to show the association of these techniques. We trained a ImageNet pretrained VGG19-based supervised learning algorithm supervised with our \typename to examine the similarities among techniques.
 }}
\label{fig:visTypesNet}
\end{figure*}https://www.overleaf.com/project/6369090010603dac989cf11b

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> supplementDatasetDrivenEvaluation.tex <==
\section{\jctg{From Point-based Evaluation to Dataset Scale Evaluation}}

\noindent

Categorization is meant to be broad, as the images only need to share their essential stimuli of the coded data. A type contains both the typical items (called prototypes) and atypical ones. We focus on a meta analysis of what representations are out there in our community (Our 7.A).

Those two papers are evaluation papers. Their techniques are specific for their evaluation purpose. Our typology can help provide the evaluators a much broader set of choices – one should look at both within and cross-category plots when choosing the charts.

For example, the first paper (Xiong et al.) could have evaluated more suitable forms of visual representations for the decision tasks (whether or not to use skin creams or carry handguns in public). The tasks require an integrated display. Bars are generally good for point reading, but unsuitable for integrating between bars for rate changes. A better statistical chart is thus not to evaluate bars, but to use more visually salient line graphs or donut charts instead. See our redraw of data in Figure 1.  Thus, the conclusion would not be generalized to “Table is better”. Lines would be better at revealing patterns. 

Another bar form, donut chart may facilitate this integrated display since the arc could be more accurate for making part/whole judgments, than the arc length itself in bars.  

In this regard, our typology certainly does not have the design principle of integrated display, as we have described here. But one may use our typology to look up more suitable forms of design. Even better, instead of point evaluations, use dataset scale evaluation instead. Our community may use our typology to summarize principles between and within categories for education uses of ones’ visual literacy.

The second paper (Newburger et al.) evaluated four charts that can be conveniently mapped to our typology. 
Bar histogram -> area-based (our code)
Dot plot -> point-based
Boxplot -> bar-based and point-based
Strip plot -> bar-based 

So to evaluate these, we could potentially educate the viewers that these charts used very different essential stimuli and our typology can teach observers what information to be extracted, from these specific techniques. One may also consider if the outcomes would be reusable for techniques sharing the essential stimuli. 

We have added these two specific papers as case studies to turn point-based design to data-set based evaluation. We have also added the second paper to describe potentially generalizable design guidelines. We have credited this reviewer in our writing. 


